Transformer Networks for Trajectory Forecasting

Most recent successes on forecasting the people motion are based on LSTM models and all most recent progress has been achieved by modelling the social interaction among people and the people interaction with the scene. We question the use of the LSTM models and propose the novel use of Transformer Networks for trajectory forecasting. This is a fundamental switch from the sequential step-by-step processing of LSTMs to the only-attention-based memory mechanisms of Transformers. In particular, we consider both the original Transformer Network (TF) and the larger Bidirectional Transformer (BERT), state-of-the-art on all natural language processing tasks. Our proposed Transformers predict the trajectories of the individual people in the scene. These are "simple" model because each person is modelled separately without any complex human-human nor scene interaction terms. In particular, the TF model without bells and whistles yields the best score on the largest and most challenging trajectory forecasting benchmark of TrajNet. Additionally, its extension which predicts multiple plausible future trajectories performs on par with more engineered techniques on the 5 datasets of ETH + UCY. Finally, we show that Transformers may deal with missing observations, as it may be the case with real sensor data. Code is available at https://github.com/FGiuliari/Trajectory-Transformer.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/OLDexperiments.tex <==
\section{Experimental Evaluation}\label{Sec:exp}

\todo{Marco: please review the overall structure of this section and how this is matching the tables. Table are up-to-date, to the best of my understanding.}

\todo{Irtiza: please complete the datasets and metrics section.}

We show the capabilities of the proposed $T^2F$ Transformer Networks on two recent and large datasets: the TrajNet Challenge~\cite{sadeghiankosaraju2018trajnet} dataset and the ETH+UCY dataset~\todo{citation for eth+ucy}. Additionally, we perform ablation study to quantify the model robustness against the widely-adopted LSTM. Furthermore, we analyze the effect of data augmentation (random scaling and rotation) and regression Vs.\ classification in the TF network.
Finally we illustrate the confidence of $T^2F$.
In addition, we focus here for the first time to the problem of missing data, occurring when some observation samples are missing due frame-rate drop or excessive uncertainty in the tracking data.




\subsection{Datasets and Metrics}

\todo{Irtiza: please complete}

\subsubsection{TrajNet Dataset~\cite{sadeghiankosaraju2018trajnet}} The TrajNet benchmark...

\todo{Irtiza: please complete}

\subsubsection{ETH+UCY dataset~\todo{citation for eth+ucy}} The ETH+UCY dataset suite...

\todo{Irtiza: please complete}

\subsubsection{Mean and Final Average Displacement Errors} Performance is evaluated...

\todo{Irtiza: please complete}



\subsection{The Trajnet Challenge}\label{sec:trajnet}

In the individual forecasting, the data taken into account refer to a specific individual trajectory, ignoring co-occurrent trajectories, both during training and testing time. 
As dataset we consider the TrajNet Challenge~\cite{sadeghiankosaraju2018trajnet}, the largest multi-scenario forecasting benchmark, since it reports the most effective individual forecasting approaches so far; the challenge requests to predict 3161 %(343+51+183+85+235+155+630+427+61+12+52+110+35+362+14+334+10+20+30+12)
human trajectories, observing for each trajectory 8 consecutive ground-truth values (3.2 seconds) \emph{i.e.}, $t-7,t-6,\ldots,t$, in world plane coordinates and forecasting the following 12 (4.8 seconds), \emph{i.e.}, $t+1,\ldots,t+12$.  TrajNet is a valid benchmark to check the model versatility: the challenge requires to train on four families of trajectories, namely 1) BIWI Hotel~\cite{pellegrini2009iccv} (orthogonal bird's eye flight view, moving people), 2) Crowds UCY \cite{lerner2007crowds} (3 datasets, tilted bird's eye view, camera mounted on building or utility poles, moving people), 3) MOT PETS~\cite{PETS2009} (multisensor, different human activities) and 4) Stanford Drone Dataset~\cite{Robicquet:230262} (8 scenes, high orthogonal bird's eye flight view, different agents as people, cars etc.), for a total of 11448 trajectories. Testing is requested on diverse partitions of BIWI Hotel, Crowds UCY, Stanford Drone Dataset, and is evaluated by the TrajNet server (ground-truth testing data is unavailable for applicants).

At the moment of writing, TrajNet is hosted on two diverse websites, reporting different approaches\footnote{\url{http://trajnet.epfl.ch/} and \url{http://trajnet.stanford.edu/}.}. For the sake of completeness, we show here the merge of the performances listed in the two websites, reporting only \emph{individual} approaches which are referred with a proper reference. In addition, we report the performances described in~\cite{becker2018evaluation}, where the authors discuss the performance of several independent forecasting algorithms. The merged results are in  Tab.~\ref{Tab:TrajNet}. All the approaches that have applied to TrajNet, including those with contextual information, will be discussed in Sec.~\ref{Sec:social}.  The results are in terms of Mean Average Displacement (MAD), Final Average Displacement (FAD) and their average, all measured in meters.  

Notably, the TrajNet absolute top approach so far, RED\_v3, is an individual forecasting approach~\cite{becker2018evaluation}, as so as \#4 (RED\_v2) and \#4 (RED) which are RNN-Encoder-MLP architectures. This shows that individual approaches can be extremely powerful in capturing arbitrarily complex dynamics. The other individual approaches range from linear interpolation to MLP, RNN and LSTM, also detailed in~\cite{becker2018evaluation}.    
%and among the competitors are the recent Social GAN~\cite{gupta2018social}, MX-LSTM (without head orientation info)~\cite{Hasan18}, SR-LSTM~\cite{zhang2019sr}, which will be considered also in the following suites of experiments. Social LSTM and derivates are only present with un-referred algorithms, and anyway are ranking low (starting from rank 23 downward)
%In addition, we show on Crowds UCY \cite{lerner2007crowds} (which allows us to drop the fixed 12-steps ahead forecasting regime) how II-TF deals successfully with a) extended prediction time horizons, b) short observation periods, c) missing data and in general variable frame-rate, representing thus one of the most versatile forecasting algorithms nowadays.  
%Here I-Tran ranks first in the challenge, and is showed to deal successfully with extended prediction time horizons, short observation periods, missing data and in general variable frame-rate, representing thus one of the most versatile forecasting algorithms nowadays. Sec.~\ref{Sec:MPE} discusses the explainability of the I-Tran by looking into its parameters, and its variability when parameters are changed. ...to be continued...
%Subsequently, the social extension S-TRAN is tested, which comes into play when multiple concurrent trajectories can be observed. Finally, S-MAP-TRAN is taken into account, when additionally semantic information on the scene is available. 


\begin{table}[t]
\begin{center}
\small
\caption{TrajNet Challenge results (World H-H TrajNet challenge) obtained by  \textbf{individual forecasting} approaches. The results have been collected by merging those retrieved on the two TrajNet websites\footnote{\url{http://trajnet.epfl.ch/} and \url{http://trajnet.stanford.edu/}}  and those presented in \cite{becker2018evaluation}. ``Rank'' indicates the absolute ranking over all the approaches including also those considering additional contextual information (TrajNet websites accessed on 11 15 2019). \vspace{-0.2cm} \label{Tab:TrajNet}}
\begin{tabular}{cllll} \toprule
    {Rank} & {Method} & {Avg} & {FAD} & {MAD} \\ \midrule
    1  & \tbf{TF (\emph{ours})} & \tbf{0.7345} & \tbf{1.119} & \tbf{0.350} \\
    2  & REDv3\cite{becker2018evaluation}(2019) & 0.7805 & 1.201  & 0.36  \\
%   3  	algortihm_FIFM %	0.7895 %	1.217 %	0.362 
    4  & REDv2\cite{becker2018evaluation}(2019) & 0.783 & 1.207  & 0.359  \\
    %5 & physical computation &0.793&	1.226&	0.36\\
    6  & RED\cite{becker2018evaluation}(2018) & 0.7975 & 1.229  & 0.366  \\
%   7  & SR-LSTM \cite{zhang2019sr} & 0.8155 & 1.261 & 0.37 \\ 
%     8 & linear_off5 & 0.8185	&1.266	&0.371\\
 %   9  & S.Forces (EWAP) \cite{helbing1995social} & 0.8185  & 1.266 & 0.371 \\
 %10 &fishy3&		0.82 &	1.265&	0.375\\
 %11 &lstm_offsets_v4_attention_sa_pa & 0.8185 &	1.256 &	0.381\\
12  & N-Lin. RNN-Enc-MLP\cite{becker2018evaluation} &  0.827&  1.276&  0.377\\
13  & N-Lin. RNN\cite{becker2018evaluation}(2018) &  0.841&  1.300 & 0.381\\
%14 &JHU Offsets MLP5 &	0.844 &	1.304 &	0.384\\
15  & Temp. ConvNet (TCN)\cite{bai2018empirical} & 0.841 &  1.301 & 0.381\\
16  & N-Linear Seq2Seq\cite{becker2018evaluation} &  0.860 & 1.331 & 0.390\\
17  & Vanilla LSTM (Off)\cite{LSTM_MATLAB}(2016)	& 0.8865&	1.374&	0.399\\
%17 & notSoStupidPredictorSUL	& 0.8865&	1.374&	0.399\\
%    18  & MX-LSTM \cite{Hasan18} & 0.887           & 1.374 & 0.399\\
%19 &  lstm_offsets_v3	&	0.8885 &	1.37 &	0.407\\
20  & Lin. RNN-Enc.-MLP\cite{becker2018evaluation} & 0.892 & 1.381 & 0.404\\
21  & Lin. Interpolation\cite{becker2018evaluation} & 0.894 & 1.359 & 0.429\\
%22 & linear simpler & 0.8895 &	1.372 &	0.407\\
23  & Lin. MLP (Off)\cite{becker2018evaluation} & 0.896 & 1.384 & 0.407\\
%    24  & S.Forces (ATTR) \cite{helbing1995social} & 0.9035  & 1.395 & 0.412 \\
%    25  & StupidPredictorSUL & 0.9035  & 1.395 & 0.412 \\
26  & Lin. Seq2Seq\cite{becker2018evaluation} & 0.923 & 1.429 & 0.418\\
27  & Gated TCN\cite{bai2018empirical} & 0.947 & 1.468 & 0.426\\
28  & Lin. RNN\cite{becker2018evaluation} & 0.951 & 1.482 & 0.420\\
%29  & sgan median	&	1.031 &	1.577 &	0.485 &
30  & Lin. MLP (Pos)\cite{becker2018evaluation} & 1.041 & 1.592 & 0.491\\
% 31 & sgan_mean	& 1.0835 &	1.662 &	0.505\\
% 32 & sgan traj dataset &	1.28 &	1.976 &	0.584\\
% 33  & S-GAN~\cite{gupta2018social} & 1.334  & 2.107 & 0.561   \\
% 34 & OSG_v3 &	1.385 &	2.106 &	0.664\\
% 35 &	social lstm_v2 &	1.3865 &	2.098 &	0.675\\
% 36 & social lstm % 	1.5625 %	2.299 %	0.826\\
37  & Gauss. Process \cite{trautman2010iros} & 1.6415           & 1.038 & 2.245\\
%38 & SLSTM v1.0	& 2.055 &	3.038 &	1.072\\
39  & N-Linear MLP (Off)~\cite{becker2018evaluation} & 2.103 & 3.181 & 1.024 \\
% 40 & vanilla_lstm &		2.107 &	3.114 &	1.1\\
% 41 & occupancy_lstm	&	2.1105 &	3.12 &	1.101\\
% 42 & S-LSTM &	2.4185 &	3.569	& 1.268\\
% 43 & social lstm_v3	& 	2.8735 &	4.323 &	1.424 \\
% 44 & lstm_offsets_2	&	7.1775 &	11.718 &	2.637\\
% 45 & InkognitoTracker2 & 17.793 &	22.293 & 13.293 \\
% 46 & InkognitoTracker &	17.8575 &	22.359	& 13.356 \\
% 47 % linear_v02 &	22.907 &	22.856 &	22.958
% 48 % CV &	23.0775	& 22.971 &	23.184\\
%
\textcolor{red}{new} & BERT~\cite{BERT19} &	0.897	& 1.354 &	0.44\\
\textcolor{red}{new} & BERT NLP-pre-tr (reg) &	0.902 & 1.357 & 0.447\\
\textcolor{red}{new} & LSTM &	1.14 & 1.793 & 0.491\\
\textcolor{red}{new} & BERT (classify) &	0.895 & 1.36 & 0.43\\
%
\bottomrule
%
\end{tabular}
\end{center}
\end{table}

Our TF has been trained with \todo{details on the model} (more details on the parameters importance in Sec.~\ref{Sec:MPE}). As visible in the table, TF ranks in first position, with a margin w.r.t REDv3 of \~0.05, where the first 10 positions have an average consecutive gap of \~0.01. On 3161 trajectories this means to diminish the global error of about 145 meters. Our BERT has been trained with \todo{details on the model} (more details on the parameters importance in Sec.~\ref{Sec:MPE}).







\todo{Marco: In what follows we have three subsubsections, regarding history, observation lengths and missing data. Please revise the drafted text, the chosen order of discussions and what to report.}


\subsubsection{Changing the Observation Lengths \label{Sec:history}}
It is important to evaluate the stability of the TF when leveraging fewer observations.
With this experiment, we seek to analyze the model capability to store and exploit memory, i.e.\ past observations, to predict the future. LSTM have often been criticized for their poor memory encoding, effectively saturating after a few frames. By contrast Transformer Networks have been reported to more effectively use long observations.

In Table~\ref{Tab:history}, we consider the TrajNet train/test setup and drop a variable number of frames, starting from the farthest in time.
%
\begin{table}[h!]
\caption{Evaluation of the $T^2F$ Vs.\ LSTM model performance on a variable number of history observations on TrajNet. Specifically, we drop observation frames, starting from the farthest, e.g.\ 3 frames dropped means dropping frames $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^{-6}_{t=-8)}$ and memorizing frames $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^{-1}_{t=-5)}$.
}
\label{Tab:history}
\begin{tabular}{lll}
\# Frames dropped & $T^2F$ (FAD/MAD)  & LSTM (FAD/MAD) \\
0 (no drop)       & 1.119 / 0.350 & 1.793 / 0.491 \\
1       & 1.32 / 0.471  & 1.713 / 0.476  \\
2       & 1.51/0.637    & 1.661 / 0.466  \\
3       & 1.72/0.81     & 1.60/ 0.45     \\
4       & 2.00 / 1.01   & 1.535. / 0.434 \\
5       & 2.31 / 1.32   & 1.485 / 0.33   \\
6       & 2.68 / 1.45   & 1.7 / 0.534  
\end{tabular}
\end{table}
%
The proposed $T^2F$ shows a plausible behavior, increasing error monotonically from 1.119 / 0.350 to 2.68 / 1.45 (MAD/FAD), when leveraging all frames or dropping 6 of those respectively. By contrast the LSTM reaches top performance when dropping 5 frames, i.e.\ 1.485/0.330 (FAD/MAD). This highlights two issues: \textbf{i.}\ LSTM is not capable of using properly longer-time horizons, as providing more observed frames degrades performance; and \textbf{ii.}\ a base performance may be achieved in the TrajNet dataset by leveraging simple assumptions or constant velocity and acceleration of walking people, since an LSTM-based model using only two frames still achieves a small error of 1.485/0.330 (FAD/MAD). The latter issue was already maintained in the RED work~\cite{red}. The proposed $T^2F$ does not pick on the simple behavior of most people and does not reach the same level of performance for the case of dropping 6 frames. On the other hand, $T^2F$ reaches best performance when 8 observations are provided, as it should correctly be. \todo{Marco: this story is weird. Should we include this too? Irtiza double-checked this twice. So it is really so.}








\subsubsection{Changing the Prediction Lengths \label{Sec:var_length}}
It is important to evaluate the stability of the TF when producing longer predictions, possibly when longer observations are available. Unfortunately, TrajNet does not allow to set up variable-length experiments, since trajectories are rigidly arranged as 8s obs.+12s pred. Therefore, motivated by their widespread and recent use as forecasting benchmarks~\cite{alahi2016cvpr,gupta2018social,sadeghian2019sophie,zhang2019sr,Hasan18}, we refer to those sequences within the ETH~\cite{pellegrini2009iccv} and UCY~\cite{lerner2007crowds} repositories which are not included into the TrajNet train set, namely on ETH-univ and UCY-zara01. We vary the observation sequence, from 12 frames (4.8s) to 32 frames (12.8) at a step of 1.8s. As comparison we evaluate the LSTM~\cite{LSTM_MATLAB}, since it is a common comparison in modern forecasting~\cite{alahi2016cvpr,gupta2018social,sadeghian2019sophie,zhang2019sr,Hasan18,becker2018evaluation}, its code is available (while ranks 2-16 of TrajNet are not), and because it is the basis element of several advanced systems \cite{alahi2016cvpr,Hasan18}. Both of the systems have been trained one-dataset-out with training sequences of 8 samples and 12 for the prediction. 

\begin{table}[h]
\footnotesize
\caption{MAD and FAD errors when letting the $T^2F$ and the LSTM models predict longer horizons, i.e.\ from 12 to 32 time steps. Both models were trained on the TrajNet train set, while errors are reported over the union of ETH and Zara1 sequences (not part of the TrajNet train set).}
 \begin{tabular}{ccc}
  \toprule
    {Pred.} & {LSTM~\cite{LSTM_MATLAB}} & {\textbf{TF (ours)}} \\ 
    {} & {MAD / FAD} & {MAD / FAD}\\\midrule
12      & \textbf{0.71/1.56} & 0.78/1.70 \\
16      & \textbf{0.95/2.15} & 1.15/2.72 \\
20      & \textbf{1.27/2.90} & 1.64/3.99 \\
24      & \textbf{1.66/3.76} & 2.29/5.55 \\
28      & \textbf{2.27/5.09} & 3.07/7.46 \\
32      & \textbf{2.98/4.52} & 4.13/9.96
\bottomrule\\
\\
\\
\end{tabular}
%
%
\label{Tab:var_length}%
\end{table}
On Table\ref{Tab:var_length} are reported the average MAD and FAD values over the ETH-univ and UCY-zara1. Obviously, performances are generally decreasing. TF has a consistent advantage at every horizon Vs.\ LSTM and the decrease with the horizon of LSTM is approximately 25\% worse, as LSTM degrades from 0.78 to 4.13 MAD, while TF degrades from 0.71 to 2.98 MAD.
%This is due to the fact that most of the trajectories are linear (especially on UCY-Zara1), and both LSTM and TF capture this aspect. Anyway, isolating the two datasets with more irregular trajectories that is ETH-Hotel~\cite{pellegrini2009iccv} (people getting on and off the tram), and  UCY-univ~\cite{lerner2007crowds} (open square with free conversational groups) and averaging their MAD and FAD gives the curves at Fig.~\ref{Fig:var_length}, where the error slope of LSTM is more than linear toward longer horizons, while Inf-FS is definitely linear. 









\subsubsection{Missing and noisy data \label{Sec:missing}}
At the best of our knowledge, the problem of having missing coordinates in \emph{coordinate-based} long-term forecasting\footnote{\emph{Coordinate-based} forecasting takes as input floor coordinates of people, and is different to \emph{image-based} forecasting, where images are processed to extract bounding boxes locations on the image plane such as~\cite{kitani2012activity}.}  has been never taken into account. On the contrary, the problem of missing data is common in short term-forecasting (\emph{i.e.} tracking \cite{al2011everybody}), or forecasting of heterogeneous data \cite{anava2015online,chen2001study,rodrigues2013spectral,ghazi2018robust,golyandina2007caterpillar}, where in general is treated by designing ad-hoc extensions for filling properly the missing entries (the so called \emph{hindsighting}~\cite{anava2015online}). 
Compared to these techniques, our Transformer architecture represents a novel view, since \emph{it does not need to fill missing data}; instead, it exploits the remaining samples knowing when they have been observed thanks to the positional encoding. For example, supposing the $t-k$th sample being missed in the observation sequence, the Transformer will use the remaining $t-7,\ldots,t-k-1,t-k+1,\ldots,t$, with $1\leq k \leq8$ to perform the prediction of $t+1,\ldots,t+12$. This structural ability is absent in LSTM and RNN in general (they cannot work with missing data), and in this sense the Transformer is superior. If replacements of missing values can be computed, we found that simple linear interpolation gives slight improvements to the results.

Having witnessed the superiority of the Transformer over LSTM in absolute sense (on TrajNet, see Tab.~\ref{Tab:TrajNet}) and varying the forecasting horizons (Sec.~\ref{Sec:var_length}), we continue this analysis focusing on our proposed model on the same TrajNet dataset. The idea is to systematically drop one element at observation time, at a fixed position, from the most recent (time $t$) to the furthest ($t-7$).
Results are reported in Tab.~\ref{Tab:MissingNew}.

\begin{table}[t]
\begin{center}
\small
\caption{Evaluation of missing data results for TF on TrajNet. We experiment dropping a varying number of most recent observed samples, either including or excluding the current frame. For example, in the case of dropping 3 frames, we drop $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^0_{t=-2)}$ and  $\mathcal{T}_{obs}=\{\mathbf{x}^{(i)}_t\}^{-1}_{t=-3)}$ respectively.
}\vspace{-0.2cm}
\label{Tab:MissingNew}
\begin{tabular}{ccc} \toprule
    {\# frames dropped} & {drop most recent obs.} & {drop most recent obs.}\\ & incl.\ current frame & excl.\ current frame\\ & ({FAD}/{MAD})& ({FAD}/{MAD})\\
    \midrule
0        & 1.119 / 0.350        & 1.119 / 0.350        \\
    \midrule
1        & 1.305/ 0.389         & 1.267 / 0.373        \\
2        & 1.409 / 0.429        & 1.29 / 0.38          \\
3        & 1.602 / 0.495        & 1.303 / 0.384        \\
4        & 1.787 / 0.557        & 1.313 / 0.387        \\
5        & 1.897/ 0.593         & 1.327 / 0.329        \\
6        & 2.128 / 0.669        & 1.377 / 0.406       
\bottomrule
\end{tabular}
\end{center}
\end{table}
The results show that, in a complex scenario such as TrajNet, dropping input frames impact the prediction performance, matching the intuition: the more dropped frames the larger the performance decrease. Interestingly, the current frame plays a key importance, as it is the most recent observed input, from which future predictions start. In fact, dropping the current frame together with the most recent 6 nearly doubles the error, i.e.\ degrades performance by 91\%, from 0.350 to 0.669 MAD. By contrast dropping 6 observed frames but keeping the current one only degrades the performance by 16\% (from 0.350 to 0.406 MAD), although the TF may now only leverage 2 observations (farther and closest in time).










\subsubsection{Transformer Network Model Parameter Exploration}\label{Sec:MPE}
Here we explore aspects of the Transformer Network model concerning data augmentation (random rotation, random scaling) and regression Vs.\ classification.

\todo{Marco, for your consideration: we would have a table comparing the two data augmentation policies (random scale and rotation) on TF and BERT, on trajnet. Here we could also gather the regression Vs classification results.}










\subsection{ETH+UCY datasets}

Motivated by their widespread and recent use as forecasting benchmarks~\cite{alahi2016cvpr,gupta2018social,sadeghian2019sophie,zhang2019sr,Hasan18}, we now turn to the ETH~\cite{pellegrini2009iccv} and UCY~\cite{lerner2007crowds} repositories, further organized in 5 datasets: ETH-univ, ETH-hotel, UCY-zara01,
UCY-zara02 and UCY-univ. 

\subsubsection{Single future outcome prediction}

First off we compare against individual models predicting single future outcomes.

\begin{table}[h]
\begin{tabular}{l|l|ll|llll}
        & Linear    & \multicolumn{2}{l|}{LSTM-based} & \multicolumn{4}{l}{Ours TF-based}                \\
Dataset & Linear    & LSTM          & S-GAN (1V-1)    & TF          & TF-class  & BERT      & BERT-class \\
Eth     & 1.33/2.94 & 1.09/2.94     & 1.13/2.21       & 1.03 / 2.10 & 1.01/2.13 & 1.00/2.06 & 1.02/2.18  \\
Hotel   & 0.39/0.72 & 0.86/1.91     & 1.01/2.18       & 0.47/1.05   & 0.3/0.55  & 0.24/0.44 & 0.29/0.58  \\
Ucy-uni & 0.82/1.59 & 0.61/1.31     & 0.60/1.28       & 0.53/1.32   & 0.57/1.23 & 0.69/1.39 & 0.67/0.42  \\
Zara1   & 0.62/1.21 & 0.41/0.88     & 0.42/0.91       & 0.44/1.00   & 0.44/0.97 & 0.55/1.11 & 0.45/0.98  \\
Zara2   & 0.77/1.48 & 0.52/1.11     & 0.52/1.11       & 0.34/0.76   & 0.33/0.74 & 0.42/0.84 & 0.34/0.75  \\
Avg     & 0.79/1.59 & 0.70/1.52     & 0.74/1.54       & 0.56/1.25   & 0.53/1.12 & 0.58/1.17 & 0.55/0.98 
\end{tabular}
\end{table}

\todo{To be written and commented}



\subsubsection{Multiple future outcome predictions}

Here we compare against models predicting multiple future outcomes.

We also compare our TF against the most recent social approaches of Social-LSTM~\cite{alahi2016cvpr}, Social-GAN~\cite{gupta2018social}, Sophie~\cite{sadeghian2019sophie}, SR-LSTM~\cite{zhang2019sr}. SoPhie has one of the highest performance, but the code is not available, so we refer to their results published in the original paper, and we consider the same benchmarks for a fair comparison. In particular, we consider the 2 public pedestrian walking benchmarks, ETH~\cite{pellegrini2009iccv} and UCY~\cite{lerner2007crowds}, which break down in 5 datasets: ETH-univ, ETH-hotel, UCY-zara01,
UCY-zara02 and UCY-univ.    

\todo{more to be written.}

\begin{table}[h]
\caption{Comparison against state of the art models, all predicting social and multiple futures and all based on LSTM. Ours predicts multiple futures but does not leverage social information}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|lllllll|l}
        & \multicolumn{3}{l}{Social models (LSTM-based)}                    & \multicolumn{4}{l|}{Social and mult. future (LSTM-based)} & Ours w/o social part (TF-based) \\
Dataset & Soc LSTM  & Soc Attention & \multicolumn{1}{l|}{Trajectr.++ (MM)} & S-GAN (20V-20)  & S-GAN      & Trajectron++  & Soc.-BIGAT & MM Qz TF                        \\
Eth     & 1.09/2.35 & 0.39/3.74     & \multicolumn{1}{l|}{0.50/1.19}        & 0.81/1.52       & 0.87/1.62  & 0.35/0.77     & 0.69/1.29  & 0.61 / 1.12                     \\
Hotel   & 0.79/1.76 & 0.29/2.64     & \multicolumn{1}{l|}{0.24/0.59}        & 0.72/1.61       & 0.67/1.37  & 0.18/0.38     & 0.49/1.01  & 0.18 / 0.30                     \\
Ucy-uni & 0.67/1.40 & 0.20/0.52     & \multicolumn{1}{l|}{0.36/0.89}        & 0.60/1.26       & 0.76/1.52  & 0.22/0.48     & 0.55/1.32  & 0.35 / 0.65                     \\
Zara1   & 0.47/1.00 & 0.30/2.13     & \multicolumn{1}{l|}{0.29/0.72}        & 0.34/0.69       & 0.35/0.68  & 0.14/0.28     & 0.30/0.62  & 0.22 / 0.38                     \\
Zara2   & 0.56/1.17 & 0.33/3.92     & \multicolumn{1}{l|}{0.27/0.67}        & 0.42/0.84       & 0.42/0.84  & 0.14/0.30     & 0.36/0.75  & 0.17 / 0.32                     \\
Avg     & 0.72/1.54 & 0.30/2.59     & \multicolumn{1}{l|}{0.34/0.84}        & 0.58/1.18       & 0.61/1.21  & 0.21/0.45     & 0.48/1.00  & 0.31 / 0.55                    
\end{tabular}
} %resizebox
\end{table}













%Illustration and analysis of self attention (the possibility of looking at importance of vislet, tracklet, etc. -> explainable.

\todo{Irtiza: Illustration of qualitative results: our best Vs LSTM, our failures Vs successes of LSTM.}

\todo{Francesco, Marco: Illustration of confidence: our TF-classify Vs LSTM with Gaussian predictions.}










==> sections/SuppMat.tex <==
\newpage
\clearpage

\section{Supplementary material}

Here we paste the experiments which we have decided to not include into the paper, but ``may'' get into the supplementary material.

\todo{Include here the correct one table for the varying horizon, as the experiments\_old.tex file contains multiple versions.}


\begin{table}[b]
  \centering
  \caption{Mean Average Displacement (MAD) error when changing the observation interval. Forecasting horizon is kept constant at 12 frames. \todo{This table should probably be omitted.}}
  \label{table:table3Ab}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|l||l|l|}
    \hline
    Dataset & Prediction interval & Vanilla LSTM & Individual TF\\
    \hline \hline
    \multirow{3}{*}{\vspace{-1em}\textbf{Eth}} &
    \textbf{Obs = 8} & 0.61 / 1.20 & 0.62 / 1.24\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.58 / 1.16 & 0.65 / 1.31\\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.59 / 1.18 & 0.65 / 1.25\\
    
    \hline \hline
    \multirow{3}{*}{\vspace{-1em}\textbf{Hotel}} &
    \textbf{Obs = 8} &  0.53 / 1.13 & 0.34 / 0.66\\
    \cline{2-4}
    & \textbf{Obs = 12} & 0.36 / 0.73 &  0.32 / 0.61\\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.29 / 0.55 & 0.26 / 0.45\\
  
    \hline \hline
    \multirow{3}{*}{\vspace{-1em}\textbf{Uvy-univ}} &
    \textbf{Obs = 8} & 0.57 / 1.18 & 0.60 / 1.30\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.55 / 1.23 & 0.66 / 1.39\\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.53 / 1.19 & 0.65 / 1.25  \\
    \cline{2-4}
    \hline \hline
    \multirow{3}{*}{\vspace{-1 em}\textbf{Zara1}} &
    \textbf{Obs = 8} & 0.42 / 0.92 & 0.42 / 0.92\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.41 / 0.91 & 0.43 / 0.95\\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.41 / 0.92 & 0.47 / 1.05\\
    \cline{2-4}
    \hline \hline
    \multirow{4}{*}{\vspace{-1 em}\textbf{Zara2}} &
    \textbf{Obs = 8} & 0.35 / 0.78 & 0.34 / 0.74\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.32 / 0.72 & 0.38 / 0.85\\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.29 / 0.68 & 0.30 / 0.67\\
    \cline{2-4}
    
   
     \hline
    \end{tabular}
  }
\end{table}



\begin{table*}[t!]
\caption{Results with Social GAN data-outdated}
  \centering
  \resizebox{0.9\linewidth}{!}{%
  \begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l}
    \midrule
    & \multicolumn{7}{c|}{\textbf{Baselines}} & \multicolumn{5}{c}{\textbf{Social Transformer (Ours)}} \\
    \cmidrule[1pt]{2-13}
    \textbf{Dataset} & \textbf{Lin} & \textbf{LSTM} & \textbf{S-LSTM} & \textbf{S-GAN} & \textbf{S-GAN-P} & \textbf{SoPhie} & \textbf{SR-LSTM} & \textbf{TK} & $\mathbf{Tk+ DA}$ & $\mathbf{Tk+OccMaps}$ & \textbf{TK(SR-LSTM dt)} &\textbf{TK+OCC(SR-LSTM dt)}\\
    \midrule
\textbf{ETH} & 1.33 / 2.94 & 1.09 / 2.41 & 1.09 / 2.35 & 0.81 / 1.52  & 0.87 /  1.62 & 0.70 / 1.43 &\textbf{0.63 / 1.25}& 1.07 / 2.22 & 1.02 / 2,18 & 0.83 / 1.74 & 0.65 & 0.66 / 1.40\\
    \textbf{HOTEL} & 0.39 / 0.72 & 0.86 / 1.91 & 0.79 / 1.76 &  0.72 / 1.61 & 0.67 / 1.37 & 0.76 / 1.67 &0.37 / 0.74& 0.53 / 1.15 & 0.3 / 0.58 & 0.33 / 0.71 &0.34 & \textbf{0.33/ 0.73}\\
    \textbf{UNIV}  & 0.82 /  1.59 &  0.61 /  1.31 & 0.67 / 1.40 & 0.60 / 1.26 & 0.76 / 1.52 & 0.54 / 1.24& 0.51 / 1.10 & na & 0.55 / 1.19 & 0.52 / 1.11 & 0.59 / 1.27 & \textbf{0.50 / 1.14}\\
    \textbf{ZARA1} & 0.62 / 1.21 & 0.41 / 0.88 & 0.47 / 1.00 & 0.34 / 0.69 & 0.35 / 0.68 & \textbf{0.30 / 0.63} &0.41 / 0.90  & 0.41 / 0.91 & 0.45 / 0.98 & 0.36 / 0.85 &0.40 & 0.32 / 0.75\\
    \textbf{ZARA2} & 0.77 / 1.48& 0.52 / 1.11 & 0.56 /  1.17&  0.42 / 0.84 & 0.42 / 0.84 & 0.38 / 0.78 & 0.32 / 0.70  & 0.31 / 0.69 & 0.33 / 0.73 & 0.26 / 0.64 & 0.31 & \textbf{0.25 / 0.57}\\
    \toprule
    \midrule
    \textbf{AVG}   & 0.79 / 1.59 & 0.70 /  1.52  & 0.72 / 1.54 & 0.58 / 1.18 & 0.61 / 1.21 & 0.54 / 1.15 & 0.45 / 0.94&na & 0.53 / 1.13  & 0.46 / 1.01 & 0.45& \textbf{0.41 / 0.91}\\
    \toprule
  \end{tabular}
  }
\end{table*}



\begin{table*}[]
\caption{Comparison with SOTA and MX-LSTM on Mx-LSTM data \todo{include the current results of TK+vislets}}
 \resizebox{0.9\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Datasets & LTA \cite{pellegrini2009iccv}       & SF \cite{yamaguchi2011cvpr}        & Social LSTM \cite{alahi2016cvpr} & Social GAN \cite{SocialGAN18} & Indiv-Mx-LSTM \cite{Hasan18} & MX-LSTM \cite{Hasan18}   & TK         & TK + OCC \\ \hline
Univ     & 2.49/4.66 & 2.57/4.62 & 0.62/1.40   & 0.65/1.36  & 0.53/1.16     & 0.49/1.12 & 0.44//0.99 &          \\ \hline
Zara1    & 2.74/5.55 & 2.88/5.55 & 0.68/1.53   & 0.48/1.04  & 0.63/1.37     & 0.59/1.31 & 0.31/0.69  &          \\ \hline
Zara2    & 2.23/4.35 & 2.32/4.35 & 0.63/1.43   & 0.44/0.95  & 0.72/1.56     & 0.35/0.79 & 0.25/0.56  &          \\ \hline
\end{tabular}
}
\end{table*}



% \begin{table}[]
% \caption{Ablation study with MX-LSTM on Mx-LSTM data}
%  \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Datasets & Indiv-Mx-LSTM & MX-LSTM   & TK         & TK + OCC \\ \hline
% Univ     & 0.53/1.16     & 0.49/1.12 & \textbf{0.44//0.99} &          \\ \hline
% Zara1    & 0.63/1.37     & 0.59/1.31 & \textbf{0.31/0.69}  &          \\ \hline
% Zara2    & 0.72/1.56     & 0.35/0.79 & \textbf{0.25/0.56}  &          \\ \hline
% \end{tabular}
% }
% \end{table}




\begin{table}[h]
  \centering
  \caption{Mean Average Displacement (MAD) error when changing the observation interval. Forecasting horizon is kept constant at 12 frames. \todo{Irtiza: calculate for the lstmon sgan dt}
  \label{table:table3Ab}
  
    \begin{tabular}{|l|l||l|l|}
    \hline
    Dataset & Prediction interval & Vanilla LSTM & TF-class (epoch 40)\\
    \hline \hline
    \multirow{3}{*}{\vspace{-1em}\textbf{Eth}} &
    \textbf{Obs = 8} & 0.61 / 1.20 & 1.01 /2.13\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.58 / 1.16 & na\\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.59 / 1.18 & 0.97 / 1.92\\
    
    \hline \hline
    \multirow{3}{*}{\vspace{-1em}\textbf{Hotel}} &
    \textbf{Obs = 8} &  0.53 / 1.13 & 0.3 / 0.55\\
    \cline{2-4}
    & \textbf{Obs = 12} & 0.36 / 0.73 &  na \\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.29 / 0.55 & 0.20 / 0.35\\
  
    \hline \hline
    \multirow{3}{*}{\vspace{-1em}\textbf{Ucy-univ}} &
    \textbf{Obs = 8} & 0.57 / 1.18 & 0.57 / 1.23\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.55 / 1.23 & na \\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.53 / 1.19 & \\ 0.68 / 1.4
    \cline{2-4}
    \hline \hline
    \multirow{3}{*}{\vspace{-1 em}\textbf{Zara1}} &
    \textbf{Obs = 8} & 0.42 / 0.92 & 0.42 / 0.92\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.41 / 0.91 & na \\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.41 / 0.92 & 0.43 / 0.98\\
    \cline{2-4}
    \hline \hline
    \multirow{4}{*}{\vspace{-1 em}\textbf{Zara2}} &
    \textbf{Obs = 8} & 0.35 / 0.78 & 0.33 / 0.74\\
    \cline{2-4}
    &\textbf{Obs = 12} & 0.32 / 0.72 & na \\
    \cline{2-4}
    & \textbf{Obs = 16} & 0.29 / 0.68 &  0.27/0.58\\
    \cline{2-4}
    
   
     \hline
    \end{tabular}
  
\end{table}
